QE-BEV: Query Evolution for Bird's Eye View Object Detection in Varied Contexts

3D object detection plays a pivotal role in autonomous driving and robotics, demanding precise interpretation of Bird's Eye View (BEV) images. The dynamic nature of real-world environments necessitates the use of dynamic query mechanisms in 3D object detection to adaptively capture and process the complex spatio-temporal relationships present in these scenes. However, prior implementations of dynamic queries have often faced difficulties in effectively leveraging these relationships, particularly when it comes to integrating temporal information in a computationally efficient manner. Addressing this limitation, we introduce a framework utilizing dynamic query evolution strategy, harnesses K-means clustering and Top-K attention mechanisms for refined spatio-temporal data processing. By dynamically segmenting the BEV space and prioritizing key features through Top-K attention, our model achieves a real-time, focused analysis of pertinent scene elements. Our extensive evaluation on the nuScenes and Waymo dataset showcases a marked improvement in detection accuracy, setting a new benchmark in the domain of query-based BEV object detection. Our dynamic query evolution strategy has the potential to push the boundaries of current BEV methods with enhanced adaptability and computational efficiency. Project page: https://github.com/Jiawei-Yao0812/QE-BEV

==> figures/clustering.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
    \begin{minipage}{0.5\columnwidth}
        \centering
        \fontsize{6pt}{8pt}\selectfont
        \begin{tabular}{l|cc}
        \hline
        Temporal Resolution & NDS & mAP \\
        \hline
        Every Frame & 55.5 & 44.8 \\
        Every 2 Frames  & 55.9 & 45.1 \\
        Every 5 Frames & 55.2 & 44.5\\
        \hline
    \end{tabular}
    \caption{Performance of LTFM at different temporal resolutions.}
    \label{tab:temporal_resolutions}
    \end{minipage}%
    \begin{minipage}{0.5\columnwidth}
        \centering
        \fontsize{6pt}{8pt}\selectfont
     
    \begin{tabular}{l|cc}
        \hline
        Diversity Loss & NDS & mAP \\
        \hline
        Without & 54.4 & 43.7 \\
        With    & 55.9 & 45.1 \\
        \hline
    \end{tabular}

    \caption{Impact of Diversity Loss in feature aggregation.}
    \label{tab:diversity_loss}
    \end{minipage}
\end{table}

==> figures/nuscenes_test.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table*}[h!]
  \centering
  \caption{\textbf{Performance comparison} on nuScenes \texttt{test} split.}
  \resizebox{0.8\textwidth}{!}{
  \begin{tabular}{l|c|c|cc|ccccc}
    \toprule
    Method & Backbone & Epochs & NDS & mAP & mATE & mASE & mAOE & mAVE & mAAE \\ 
    \midrule
    DETR3D \cite{detr3d}           & V2-99 & 24 & 47.9 & 41.2 & 0.641 & 0.255 & 0.394 & 0.845 & 0.133 \\
    PETR \cite{petr}               & V2-99 & 24 & 50.4 & 44.1 & 0.593 & 0.249 & 0.383 & 0.808 & 0.132 \\
    UVTR \cite{uvtr}               & V2-99 & 24 & 55.1 & 47.2 & 0.577 & 0.253 & 0.391 & 0.508 & 0.123 \\
    BEVFormer \cite{bevformer}     & V2-99 & 24 & 56.9 & 48.1 & 0.582 & 0.256 & 0.375 & 0.378 & 0.126 \\
    BEVDet4D \cite{bevdet4d}       & Swin-B \cite{swin} & 90$^\ddagger$ & 56.9 & 45.1 & 0.511 & 0.241 & 0.386 & 0.301 & 0.121 \\
    PolarFormer \cite{polarformer} & V2-99 & 24 & 57.2 & 49.3 & 0.556 & 0.256 & 0.364 & 0.440 & 0.127 \\
    PETRv2 \cite{petrv2}           & V2-99 & 24 & 59.1 & 50.8 & 0.543 & 0.241 & 0.360 & 0.367 & 0.118 \\
    Sparse4D \cite{sparse4d}       & V2-99 & 48 & 59.5 & 51.1 & 0.533 & 0.263 & 0.369 & 0.317 & 0.124 \\
    BEVDepth \cite{bevdepth}       & V2-99 & 90$^\ddagger$ & 60.0 & 50.3 & 0.445 & 0.245 & 0.378 & 0.320 & 0.126 \\
    BEVStereo \cite{bevstereo}     & V2-99 & 90$^\ddagger$ & 61.0 & 52.5 & 0.431 & 0.246 & 0.358 & 0.357 & 0.138 \\
    SOLOFusion \cite{solofusion}   & ConvNeXt-B \cite{convnext} & 90$^\ddagger$ & 61.9 & 54.0 & 0.453 & 0.257 & 0.376 & 0.276 & 0.148 \\
    %\rowcolor{Gray}
    SparseBEV~\cite{sparsebev}             & V2-99 & 24 & 62.7 & 54.3 & 0.502 & 0.244 & 0.324 & 0.251 & 0.126 \\
    
    %\textbf{SparseBEV} (dual-branch)~\cite{sparsebev} & V2-99 & 24 & 63.6 & 55.6 & 0.485 & 0.244 & 0.332 & 0.246 & 0.117 \\
    \rowcolor{Gray}
    \textbf{QE-BEV} & V2-99 & 24 & \textcolor{blue}{\textbf{65.7}} & \textcolor{blue}{\textbf{59.2}} & 0.326 & 0.261 & 0.293 & 0.252 & 0.183 \\
    %\rowcolor{Gray}
    %\textbf{QE-BEV} $\dagger$ & V2-99 & 24 & 65.8 & 57.8 & 0.481 & 0.241 & 0.334 & 0.239 & 0.114 \\
    % \midrule
    % BEVFormerV2 $\dagger$ \cite{bevformerv2} & InternImage-XL \cite{internimage} & 24 & 64.8 & 58.0 & 0.448 & 0.262 & 0.342 & 0.238 & 0.128 \\
    % BEVDet-Gamma $\dagger$ \cite{bevpoolv2}  & Swin-B & 90$^\ddagger$ & 66.4 & 58.6 & 0.375 & 0.243 & 0.377 & 0.174 & 0.123 \\
    
    % \textbf{SparseBEV} $\dagger$~\cite{sparsebev}    & V2-99 & 24 & 67.5 & 60.3 & 0.425 & 0.239 & 0.311 & 0.172 & 0.116 \\
    % \rowcolor{Gray}
    % \textbf{QE-BEV} $\dagger$             &  &  &  & &  &  &  &  &  \\
    \bottomrule
  \end{tabular}
 }

  \label{table:nuscenes_test}
\end{table*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


